Mambular: A Sequential Model for Tabular Deep Learning

The analysis of tabular data has traditionally been dominated by gradient-boosted decision trees (GBDTs), known for their proficiency with mixed categorical and numerical features. However, recent deep learning innovations are challenging this dominance. This paper investigates the use of autoregressive state-space models for tabular data and compares their performance against established benchmark models. Additionally, we explore various adaptations of these models, including different pooling strategies, feature interaction mechanisms, and bi-directional processing techniques to understand their effectiveness for tabular data. Our findings indicate that interpreting features as a sequence and processing them and their interactions through structured state-space layers can lead to significant performance improvement. This research underscores the versatility of autoregressive models in tabular data analysis, positioning them as a promising alternative that could substantially enhance deep learning capabilities in this traditionally challenging area. The source code is available at https://github.com/basf/mamba-tabular.

==> xgb_comparison.tex <==
\paragraph{Comparison to XGBoost}
When benchmarked against XGBoost using default hyperparameter settings, Mambular demonstrates comparable, if not slightly superior performance.
It significantly outperforms XGBoost on 4 out of 12 datasets at the 10\% significance level, while XGBoost surpasses Mambular on 2 datasets at the same significance level.
The $p$-values from simple t-tests over the folds are reported for each dataset with testing methodology based on \cite{gorishniy2021revisiting}
After adjusting for multiple testing via Benjamini-Hochberg \citep{ferreira2006benjamini, benjamini1995controlling} the Abalone results - only significant at the 10\% level with standard testing - are not significant anymore. All other results remain unchanged\footnote{Due to the small sample sizes, Benjamini-Hochberg is preferred to the conservative Bonferroni adjustments \citep{nakagawa2004farewell}.}.




\begin{table*}[t]
    \centering
    \caption{Comparison between Mambular and XGBoost. The left tables shows regression results with average MSE values over 5 folds. The right side shows (binary) classification results with average AUC values. Significantly better values at the 5\% significance level are in green and marked bold. Significantly better values at the 10\% significance level are underscored. Dataset details can be found in appendix \ref{app:datasets}. $\uparrow$ depicts higher is better and vice-versa. \\}
    \resizebox{\textwidth}{!}{%
    
    \begin{tabular}{l|ccccccc|ccccc}
    \toprule
          Models   & DI $\downarrow$ & AB $\downarrow$ & CA $\downarrow$ & WI $\downarrow$ & PA $\downarrow$ & HS $\downarrow$ & CP $\downarrow$ & BA $\uparrow$ & AD $\uparrow$ & CH $\uparrow$ & FI $\uparrow$ & MA $\uparrow$\\
          \hline
          Mambular & \textcolor{mygreen}{\textbf{0.018}} & \textcolor{mygreen}{\underline{0.452}} & 0.167 & 0.628 & 0.035 & 0.132 & 0.025 & 0.927 & 0.928 & \textcolor{mygreen}{\textbf{0.861}} & \textcolor{mygreen}{\textbf{0.796}} & 0.917 \\
          XGB      & 0.019 & 0.506 & 0.171 & \textcolor{mygreen}{\textbf{0.528}} & 0.036 & 0.119 & 0.024 & 0.928 & 0.929 & 0.845 & 0.774 & \textcolor{mygreen}{\textbf{0.922}} \\
          \midrule
          \footnotesize{$p$-value} & \footnotesize{0.0079} & \footnotesize{0.0870} & \footnotesize{0.4865} & \footnotesize{1.3e-07} &  \footnotesize{0.6287} & \footnotesize{0.3991} & \footnotesize{0.1999} & \footnotesize{0.7883} & \footnotesize{0.7930} & \footnotesize{0.0192} & \footnotesize{0.0120} & \footnotesize{0.010} \\
    \end{tabular}
    }
    
    \label{tab:xgb}
\end{table*}
